Spatial-Temporal Alignment Network for Action Recognition and Detection

This paper studies how to introduce viewpoint-invariant feature representations that can help action recognition and detection. Although we have witnessed great progress of action recognition in the past decade, it remains challenging yet interesting how to efficiently model the geometric variations in large scale datasets. This paper proposes a novel Spatial-Temporal Alignment Network (STAN) that aims to learn geometric invariant representations for action recognition and action detection. The STAN model is very light-weighted and generic, which could be plugged into existing action recognition models like ResNet3D and the SlowFast with a very low extra computational cost. We test our STAN model extensively on AVA, Kinetics-400, AVA-Kinetics, Charades, and Charades-Ego datasets. The experimental results show that the STAN model can consistently improve the state of the arts in both action detection and action recognition tasks. We will release our data, models and code.

==> junwei/intro.tex <==

% moved figure to main.tex
% Junwei edited - 11/14/2019;added more background and references
\section{Introduction}



% why do we need viewpoint invariant models
Humans can recognize actions from different viewpoints. However, current action recognition and detection models are sensitive to viewpoint changes and susceptible to adversarial attacks~\cite{tramer2017ensemble}, which indicates a mismatch between current action models and how humans actually perceive actions.
Meanwhile, traditional convolutional neural networks are not designed to be viewpoint-equivariant~\cite{kosiorek2019stacked}\llcao{this claim is a bit too vague for those did not read Hinton's paper. I plan to expand this part if you agree}, suggesting the need to develop a new model that could produce consistent feature representations despite viewpoint changes.
This quality is especially important for action recognition and detection for moving cameras, as they usually include viewpoint changes and ego-motions.

\llcao{what is limitation of Slowfast?}

Inspired by the Spatial Transformer Network~\cite{jaderberg2015spatial} \llcao{Zisserman's work was named earlier than transformer, but not interested } and Stacked Capsule Autoencoder ~\cite{kosiorek2019stacked} \llcao{it will be worth to explain these two methods in more details and their pros/cons}for image recognition, we propose Focal Transformer Network (FTN) \llcao{I am not sure whether we shall use the transformer as part of our model since there will be more and more `transformer' works by the end of this year. } \xuehan{rename to ``spatial temporal alignment network"} that aims to learn viewpoint invariant representations for action recognition and action detection. 
As shown in Fig.~\ref{fig:ftn}, we develop a Focal Transformer Network (FTN) Block, which takes a spatial-temporal feature input tensor, extract viewpoint invariant hints, and outputs a spatial-temporal transformation matrix for feature warping that produces an output tensor of the same shape.


\begin{figure*}[ht]
	\centering
		\includegraphics[width=0.95\textwidth]{figures/ftn.png} 
	\caption{Focal transformer network (FTN) block design.}
	\label{fig:ftn}
\end{figure*}


The FTN block is very light-weighted and generic, which could be plugged into existing action recognition models like 3D-Resnet, Non-Local Network~\cite{wang2018non} and the Slowfast network~\cite{feichtenhofer2019slowfast}. 
In Fig.~\ref{fig:ftn_arch}, as a preliminary experiment, we put FTN block between Res-1 and Res-2 in 3D ResNet architecture, and the same on the Fast pathway in SlowFast model.
For the Slowfast+FTN model, the FLOPS increase is only 1.8\% (134.04 gFLOPS vs. 131.67 gFLOPS).

\begin{figure}[ht]
	\centering
		\includegraphics[width=0.47\textwidth]{figures/ftn_arch.png} 
	\caption{Focal transformer network (FTN) block in 3D ResNet and SlowFast Network.}
	\label{fig:ftn_arch}
\end{figure}




==> related_work.tex <==
\section{Related Work}


%\cite{jaderberg2015spatial}'s work: we did temporal grouping (not totally verified); blocks;  parameterization/warping? design; 
%- hinton's 
%only video: ucf's work


%resnet3d, slowfast
%attention-based method: like alignment; action transformer (better than AVA-Kinectics, but different backbone)
%non-local network: no alignment, just transformer without feedforward, only query key value

% 1. attention
%non-local neural networks
%Video Action Transformer Network
% 2. graph
%Videos as Space-Time Region Graphs
%Graph-Based Global Reasoning Networks
%Learning Human-Object Interactions by Graph Parsing Neural Networks
%A Structured Model For Action Detection
% 3. proposal base
%R-C3D: Region Convolutional 3D Network for Temporal Activity Detection
%Rethinking the Faster R-CNN Architecture for Temporal Action Localization
%Tube Convolutional Neural Network (T-CNN) for Action Detection in Videos
% 4. optical flow-based
%Quo Vadis, Action Recognition? A New Model and the Kinetics Dataset
%Two-Stream Convolutional Networks for Action Recognition in Videos
% 5. new conv
%Trajectory Convolution for Action Recognition
%A Closer Look at Spatiotemporal Convolutions for Action Recognition
%TSM: Temporal Shift Module for Efficient Video Understanding
%SLOWFAST
%Temporal Pyramid Network for Action Recognition



\textbf{Spatial-Temporal Modeling for Actions.}
Many works~\cite{feichtenhofer2019slowfast,wang2018non,carreira2017quo} have been proposed for action recognition and detection. 
Attention-based methods~\cite{wang2018non,girdhar2019video} utilize spatial-temporal attention mechanism to capture important features for action recognition.
Many works~\cite{wang2018videos,chen2019graph,qi2018learning,zhang2019structured} have studied using graph representation to model spatial-temporal relationships between human and objects for action recognition and detection.
Inspired by Faster-RCNN~\cite{ren2015faster} in object detection, other works~\cite{xu2017r,chao2018rethinking,hou2017tube} have explored using proposal-based, two-stage models for action detection.
Optical-flow-based methods~\cite{carreira2017quo,simonyan2014two} have been proposed to focus on temporal modeling for action recognition.
Recently, many new neural networks~\cite{tran2018closer,zhao2018trajectory,lin2019tsm,feichtenhofer2019slowfast,yang2020temporal} have studied variations of convolutional models for efficient spatial-temporal modeling of actions.

% 1. capsules
%Dynamic Routing Between Capsules
%Stacked Capsule Autoencoders
%3D Point Capsule Networks
%VideoCapsuleNet: A Simplified Network for Action
% 2. viewpoint-invariant network
% 2.1 object recognition
%Spatial Transformer Networks
%Equivariant Transformer Network
%Inverse Compositional Spatial Transformer Networks
%Equivariant Multi-View Networks
% 2.2 actions
%Part-aligned pose-guided recurrent network for action recognition

%\textbf{Viewpoint-Invariant Feature Representations.}
\textbf{Capsule Network.}
As mentioned in ~\cite{sabour2017dynamic}, modern convolutional neural networks (CNNs) is susceptible to viewpoint changes and may not be optimal for object and action recognition.
Sabour et. al~\cite{sabour2017dynamic} proposed capsule networks to model viewpoint invariant representations for object recognition. 
Many follow-up works have studied capsule network for object recognition~\cite{kosiorek2019stacked}, 3D reconstruction~\cite{zhao20193d} and action recognition~\cite{duarte2018videocapsulenet}.

\textbf{pose-guided network, Skeleton-Based}
Huang et. al~\cite{huang2019part} proposed to utilize human pose information for perspective transformation for action recognition.


\textbf{Viewpoint-Invariant Feature Representations.}
Other works~\cite{jaderberg2015spatial,tai2019equivariant,lin2017inverse} have studied perspective transformation networks to improve CNN's ability to handle viewpoint changes for object recognition. All these works are for 2D image only. However, in this paper we believe that invariant based method is more crucial in spatial-temporal space, and develop a new approach that can outperform the state-of-the-art in action recognition.

% https://arxiv.org/pdf/1506.02025.pdf

% https://openaccess.thecvf.com/content_cvpr_2017/papers/Lin_Inverse_Compositional_Spatial_CVPR_2017_paper.pdf

% https://arxiv.org/pdf/1901.11399.pdf
